A Solver for a Theory of Strings and Bit-vectors

We present a solver for a many-sorted first-order quantifier-free theory $T_{w,bv}$ of string equations, string length represented as bit-vectors, and bit-vector arithmetic aimed at formal verification, automated testing, and security analysis of C/C++ applications. Our key motivation for building such a solver is the observation that existing string solvers are not efficient at modeling the string/bit-vector combination. Current approaches either reduce strings to bit-vectors and use a bit-vector solver as a backend, or model bit-vectors as natural numbers and use a solver for the combined theory of strings and natural numbers. Both these approaches are inefficient for different reasons. Modeling strings as bit-vectors destroys structure inherent in string equations thus missing opportunities for efficiently deciding such formulas, and modeling bit-vectors as natural numbers is known to be inefficient. Hence, there is a clear need for a solver that models strings and bit-vectors natively. Our solver Z3strBV is a decision procedure for the theory $T_{w,bv}$ combining solvers for bit-vector and string equations. We demonstrate experimentally that Z3strBV is significantly more efficient than reduction of string/bit-vector constraints to strings/natural numbers. Additionally, we prove decidability for the theory $T_{w,bv}$. We also propose two optimizations which can be adapted to other contexts. The first accelerates convergence on a consistent assignment of string lengths, and the second, dubbed library-aware SMT solving, fixes summaries for built-in string functions (e.g., {\tt strlen} in C/C++), which Z3strBV uses directly instead of analyzing the functions from scratch each time. Finally, we demonstrate experimentally that Z3strBV is able to detect nontrivial overflows in real-world system-level code, as confirmed against 7 security vulnerabilities from CVE and Mozilla database.

==> evalCVECaseStudy.tex <==
\smallskip
\smallskip

\noindent
\textit{Case Study}. 
\subsection{CVE Exploit Synthesis}

We performed a review of heap overflow vulnerabilities identified in
string-manipulating programs in the Common Vulnerabilities and
Exposures (CVE)
\cite{cveSite} database. We found that the primary reason for heap overflow bugs
was overflow or underflow in arithmetic computations on buffer size. Therefore,
we are interested in modelling such vulnerabilities in the theory of
strings and bitvectors and determining whether our solver is able to produce
a payload that triggers the bug. To demonstrate the efficacy of this
theory combination, we selected seven real vulnerabilities from the CVE database.
For the examples discussed here, we analyzed the vulnerable part of the code
manually and expressed path constraints in the SMTLIB2 \cite{BarFT-RR-15}
format. We created two versions of these constraints: one over strings and bitvectors,
solved using our enhanced version of Z3str2+BV,
and the second over strings and integers, which is solved using Z3str2 and compared
with the bitvector result.

\subsubsection{Google Stagefright Vulnerabilities}

The \textit{Stagefright} vulnerability refers to a bug that lives
fairly deep inside the Android operating system. Stagefright is a
system service for Android implemented in native C++ that handles
multiple media formats. The vulnerability exists due to a number of
integer overflows and underflows that lead to code injection attacks.
We briefly explain the exploit and proceed with modelling and
analyzing the vulnerable region in the following paragraphs.  To
trigger the vulnerability, an attacker sends a multimedia message
(MMS) containing a media file with an embedded payload to any
messenger application that can process the provided media file. The
Stagefright library is used for generating thumbnails as well as
playing media files, and consequently, when the thumbnail of the
malicious media file is rendered, the vulnerability can be triggered.

\begin{figure}[!t]
\centering
\begin{verbatim}[fontsize=\small]
    status_t MPEG4Source::parseChunk(off64_t *offset) {
      ...
      uint64_t chunk_size = ntohl(hdr[0]);
      uint32_t chunk_type = ntohl(hdr[1]);
      off64_t data_offset = *offset + 8;
      if (chunk_size == 1) {
        if (mDataSource->readAt(*offset + 8, &chunk_size, 8) < 8) {
          return ERROR_IO;
        }
      chunk_size = ntoh64(chunk_size);
      ...
      case FOURCC('t', 'x', '3', 'g'):
      {
        uint32_t type;
        const void *data;
        size_t size = 0;
        if (!mLastTrack->meta->findData(
                kKeyTextFormatData, &type, &data, &size)) {
          size = 0;
        }
        uint8_t *buffer = new (std::nothrow) uint8_t[size + chunk_size];
        if (buffer == NULL) {
          return ERROR_MALFORMED;
        }
        if (size > 0) {
          memcpy(buffer, data, size);
        }
        ...
    }
\end{verbatim}
\caption{Stagefright tx3g MP4 atom integer overflow}
\label{lst:stagefright-tx3g}
\end{figure}

\subsubsection{CVE-2015-3824: Google Stagefright 'tx3g' MP4 Atom Integer Overflow Remote Code Execution}

The first benchmark models a vulnerability associated with Stagefright's handler for the
\texttt{tx3g} atom in MP4 file processing. The vulnerable fragment of the handler
is shown in Figure~\ref{lst:stagefright-tx3g}. Here, the size of a dynamically-created
buffer is computing by adding together several integer variables, some of which
are controlled by the user. The values of the user-controlled variables can be selected
to cause an integer overflow that leads to a heap overflow. Analyzing the erroneous code fragment,
we can see that the size is guaranteed to be greater than zero when
\verb|mLastTrack->meta->findData()| returns \texttt{true}. The
\texttt{new} operator creates a buffer using the sum of \texttt{size} and \texttt{chunk\_size}
as its parameter. The value of \texttt{chunk\_size} is read from a file and interpreted
as a \texttt{uint64} variable. However, the argument to \verb|operator new|
is specified to be a value of type \texttt{size\_t}, the size of which varies according to the underlying
processor architecture. This leads to two different possibilities.
On a 32-bit architecture, \texttt{size\_t} is a 32-bit word, and the result is truncated to 32 bits,
which causes integer overflow. On a 64-bit architecture, \texttt{size\_t} is 64 bits,
and an enormous value for \texttt{chunk\_size} can lead to arithmetic overflow.
In either scenario, the integer overflow leads to the creation of a very small buffer on the heap,
one that is too small to hold the contents of \texttt{data}. This immediately results
in an exploitable heap overflow vulnerability triggered by \texttt{memcpy}.
We abstracted the program state and manually encoded the path constraints for this vulnerability
in the SMTLIB2 format. Solving the constraints in the theory of strings plus bitvectors
successfully produced a satisfying assignment that triggered the vulnerability.
However, solving the constraints in the theory of strings plus integers failed
to produce a model.

\subsubsection{CVE-2015-3826: Google Stagefright 3GPP Metadata Buffer Overread}

The second Stagefright vulnerability we analyze is associated with the \texttt{covr}
atom that contains album cover art. The vulnerable fragment of code is shown in
Figure~\ref{lst:stagefright-covr}. If the value of \texttt{chunk\_data\_size}
is equal to \texttt{SIZE\_MAX}, an integer overflow will occur, causing a small buffer to
be allocated. The subsequent call to \texttt{readAt} will overwrite memory locations
beyond the buffer, leading to a heap overflow. 
We encoded the path constraints for this vulnerability in the SMTLIB2 format
and solved using Z3str2; the string-bitvector solver produced a satisfying input
while the string-integer solver failed to find a model.

\begin{figure}[!th]
\centering
\begin{verbatim}
status_t MPEG4Source::parseChunk(off64_t *offset) {
  ...
  off64_t chunk_data_size = *offset + chunk_size - data_offset;
  ...
  switch(chunk_type) {
  ...
  case FOURCC('c', 'o', 'v', 'r'):
  {
    *offset += chunk_size;
    if (mFileMetaData != NULL) {
      ALOGV("chunk_data_size = %lld and data_offset = %lld",
              chunk_data_size, data_offset);
      sp<ABuffer> buffer = new ABuffer(chunk_data_size + 1);
      if (mDataSource->readAt(data_offset, buffer->data(), 
                     chunk_data_size) != (ssize_t)chunk_data_size) {
        return ERROR_IO;
      }
      ...
   ...
}
\end{verbatim}
\caption{Stagefright 3GPP metadata buffer overread}
\label{lst:stagefright-covr}
\end{figure}

\subsubsection{CVE-2009-0585: libsoup Integer Overflow}

libsoup is a library that provides HTTP client-server routines for GNOME.
An integer overflow in the \texttt{soup\_base64\_encode} function
in \texttt{soup-misc.c}, present in libsoup 2.x.x before 2.2.98
and in 2.x before 2.24, allows attackers to perform code injection via
a long string that is converted to Base64 representation.
The vulnerable part of the source code is shown in Figure~\ref{fig:libsoup}.
The \texttt{g\_malloc} function allocates heap memory using a size
that is calculated by a user-supplied, platform-specific value.
In the method, the integer \texttt{len} can overflow prior to memory allocation.
Because of this, if a large user-provided input is passed to the function,
an insufficient amount of memory is allocated, resulting in a heap-based buffer
overflow with the Base64-encoded data.
Our solver for strings plus bitvectors was able to generate a satisfying
model that triggered the vulnerability; the string-integer solver was
not able to solve the constraints.

\begin{figure}[!th]
\centering
\begin{verbatim}
        char *
        soup_base64_encode (const char *text, int len)
        {
            unsigned char *out;
            int state = 0, outlen,  save = 0;
        
            out = g_malloc (len * 4 / 3 + 5);
            outlen = soup_base64_encode_close ((const guchar *)text,
                                                len,
                                                FALSE,
                                                out,
                                                &state,
                                                &save);
            out[outlen] = '';
            return (char *) out;
        }

\end{verbatim}
\caption{libsoup integer overflow}
\label{lst:libsoup}
\end{figure}

\subsubsection{FreeBSD wpa\_supplicant(8) Base64 Integer Overflow}

This bug \cite{freeBsdOverflow} affects the 7.2-STABLE release of the FreeBSD operating system.
The \texttt{wpa\_supplicant} utility implements WPA key negoatiation with a wireless
authentication server. Figure~\ref{lst:freebsdwpa} shows the vulnerable code segment.
The exploit proceeds as follows. The user-controlled variable
\texttt{len} is multiplied with constant values and then assigned to \texttt{olen}. 
Further calculations are performed on \texttt{olen} to calculate the desired
buffer size. This final value of \texttt{olen} is used as the argument
to \texttt{os\_malloc}, which allocates heap memory. If \texttt{len} is a large value,
it leads to an integer overflow and subsequent heap memory corruption.
We encoded the vulnerable path for this program in the string-bitvector
and the string-integer theory combinations. The string-bitvector solver was able to synthesize
inputs that resulted in the vulnerable path being taken; the string-integer solver was not
able to produce a satisfying model.

\begin{figure}[t]
\centering
\begin{verbatim}
        unsigned char * base64_encode(const unsigned char *src, 
                                      size_t len,
                                      size_t *out_len){
            unsigned char *out, *pos;
            const unsigned char *end, *in;
            size_t olen;
            int line_len;
            olen = len * 4 / 3 + 4; /* 3-byte blocks to 4-byte */
            olen += olen / 72; /* line feeds */
            olen++; /* nul termination */
            out = os_malloc(olen);
            if (out == NULL)
                return NULL;
            ...
        }

\end{verbatim}
\caption{FreeBSD wpa\_supplicant(8) Base64 Integer Overflow}
\label{lst:freebsdwpa}
\end{figure}

\subsubsection{CVE-2009-2463: Mozilla Firefox/Thunderbird Base64 Integer Overflow}

This bug \cite{firefoxOverflow} was disclosed by Mozilla in 2009.
The issue affects the Base64 routines in versions of Mozilla Firefox prior to 3.0.12.
The vulnerability consists of an integer overflow that results in a heap overflow
in the \texttt{PL\_Base64Encode} function on some 32-bit architectures.
The vulnerable part of the source code is shown in Figure~\ref{lst:firefox}.
In the \texttt{PL\_Base64Encode} function, the variable \texttt{destLen}
is of type \texttt{PRUint32}, and its value is calculated
from an arithmetic expression involving \texttt{srclen}.
According to the Mozilla documentation, the \texttt{PRUint32} datatype is
defined as an \texttt{unsigned int} or \texttt{unsigned long}
depending on the platform. The variable \texttt{srclen} is the length 
of \texttt{src}, a user-controlled string. Therefore the value of \texttt{destLen}
is dependent on user input, and a very long \texttt{src} can cause integer overflow.
Furthermore, \texttt{destLen} is used as the argument of \texttt{PR\_MALLOC} to
allocate memory on the heap, leading to heap memory corruption.
We abstracted the program state and expressed the path constraints in the
SMTLIB2 format, attempting to generate models in both the string-integer
and string-bitvector theory. The string-integer solver failed to find
a satisfying assignment; however, the string-bitvector solver returned
a satisfying model that triggers the vulnerable path. 

\begin{figure}[!th]
\centering
\begin{verbatim}
    PR_IMPLEMENT(char *)
    PL_Base64Encode
    (
        const char *src,
        PRUint32    srclen,
        char       *dest
    )
    {
        if( 0 == srclen )
        {
            srclen = PL_strlen(src);
        }
        if( (char *)0 == dest )
        {
            PRUint32 destlen = ((srclen + 2)/3) * 4;
            dest = (char *)PR_MALLOC(destlen + 1);
            if( (char *)0 == dest )
            {
                return (char *)0;
            }
            dest[ destlen ] = (char)0; /* null terminate */
        }
     
        encode((const unsigned char *)src, srclen, (unsigned char *)dest);
        return dest;
    }
\end{verbatim}
\caption{Mozilla Firefox/Thunderbird Base64 integer overflow}
\label{lst:firefox}
\end{figure}

\subsubsection{CVE-2002-0639: Integer and Heap Overflows in OpenSSH 3.3}

An integer overflow vulnerability in OpenSSH versions 2.9.9 through 3.3
allows remote attackers to execute arbitrary code. Figure~\ref{lst:openssh}
shows the code fragment from OpenSSH 3.3, illustrating a classic integer overflow.
In the vulnerable path, the variable \texttt{nresp} stores an integer value
read from the client using the \texttt{packet\_get\_int} function.
The \texttt{packet\_get\_string} method returns a pointer to a buffer that resides on the heap
which contains a string read from the client. The value of \texttt{nresp}
can be set to an extremely large value, which causes the argument of \texttt{xmalloc} to overflow.
This results in allocation of a buffer of size 0. Subsequent loop iterations result in
memory corruption.
We encoded the path constraints in the SMTLIB2 format \todo{Sanu}{How did you deal with the loop?}
and solved them using the string-bitvector and string-integer solver.
The string-bitvector solver generated a satisfying input that triggers the bug,
while the string-integer solver failed to find a model.

\begin{figure}[!th]
\begin{verbatim}
                 ...
                	nresp = packet_get_int();
                	if (nresp > 0) {
                	 response = xmalloc(nresp*sizeof(char*));
                	 for (i = 0; i < nresp; i++)
                	  response[i] = packet_get_string(NULL);
                	}
                	...
\end{verbatim}
\caption{Integer and heap overflows in OpenSSH 3.3}
\label{lst:openssh}
\end{figure}

\subsubsection{CVE-2005-0180: Linux Kernel SCSI ioctl Integer Overflow}

\todo{Sanu}{Introduce this vulnerability a bit more explicitly.}
The primary reason for this vulnerability is the lack of sufficient sanitization
of user-controlled integer values. These integers are used as the size of a 
userspace-to-kernel memory copy operation. The vulnerable part of the code is 
shown in Figure~\ref{lst:linux-scsi-ioctl}. The \texttt{sg\_scsi\_ioctl} function
contains two signed integers, \texttt{in\_len} and \texttt{out\_len},
read from userspace. The third parameter of the \texttt{copy\_from\_user} method
has type \texttt{unsigned long}. However, the value that is passed 
when this method is called from \texttt{sg\_scsi\_ioctl}
is \texttt{in\_len}. If the value of \texttt{in\_len} is negative, casting it to an
\texttt{unsigned long} results in an extremely large positive value, resulting in memory overflow.
We encoded the path constraints in the theory of strings plus bitvectors and
were able to use our solver to find a satisfying input; however, the
string-integer solver was not able to solve the constraints on an equivalent string-integer representation.

\begin{figure}[h!]
\centering
\begin{verbatim}
    static int sg_scsi_ioctl(struct file *file, request_queue_t *q, ...){
        char *buffer = NULL;
        int bytes;
        int in_len, out_len;                    /* two integers */
        ...
        if (get_user(in_len, &sic->inlen))  /* read from user space */
                return -EFAULT;
        if (get_user(out_len, &sic->outlen))
                return -EFAULT;
        if (in_len > PAGE_SIZE || out_len > PAGE_SIZE)
                return -EINVAL;
        ...
        bytes = max(in_len, out_len);
        if (bytes) {
                buffer = kmalloc(bytes, q->bounce_gfp | GFP_USER);
                if (!buffer)
                        return -ENOMEM;
                memset(buffer, 0, bytes);
        }
        ...
        if (copy_from_user(buffer, sic->data + cmdlen, in_len))
                goto error;
        ...
   }
\end{verbatim}
\caption{Linux kernel SCSI IOCTL integer overflow}
\label{lst:linux-scsi-ioctl}
\end{figure}

